Exact quantization of multistage stochastic linear problems

We show that the multistage linear problem (MSLP) with an arbitrary cost distribution is equivalent to a MSLP on a finite scenario tree. We establish this exact quantization result by analyzing the polyhedral structure of MSLPs. In particular, we show that the expected cost-to-go functions are polyhedral and affine on the cells of a chamber complex, which is independent of the cost distribution. This leads to new complexity results, showing that MSLP is fixed-parameter tractable.

==> table/coef_can_sph.tex <==
%!TEX root=../main.tex


\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
$I$ 
& \footnotesize{$\besp{\va c^\top \indi{\va c \in -\cone(W_{I}^\top)}}$}
& $\coefc{I}^\top$
& $\tcoefc{I}^\top T$
& $\tcoefc{I}^\top h$
\\ \hline

$\{1,5\}$
& $-\frac{R}{4\pi}(\sqrt 2,2-\sqrt 2)$
& $\frac{R}{4\pi}(2-\sqrt 2,-2+2\sqrt 2)$
& $-\frac{R}{2\pi}(-1+\sqrt 2)$
& $\frac{R}{2\pi}(1-\frac{\sqrt 2}{2})$
\\ \hline

$\{2,5\}$
& $-\frac{R}{4\pi}(\sqrt 2,-2+\sqrt 2)$
& $\frac{R}{4\pi}(2-\sqrt 2,-2+2\sqrt 2)$
& $-\frac{R}{2\pi}(-1+\sqrt 2)$
& $\frac{R}{2\pi}(1-\frac{\sqrt 2}{2})$
\\ \hline

$\{4,6\}$
& $-\frac{R}{4\pi}(-2+\sqrt 2,\sqrt 2)$
& $\frac{R}{4\pi}(2-\sqrt 2,-2+2\sqrt 2)$
& $-\frac{R}{2\pi}(-1+\sqrt 2)$
& $\frac{R}{2\pi}(1-\frac{\sqrt 2}{2})$
\\ \hline


$\{1,6\}$
& $-\frac{R}{4\pi}(2-\sqrt 2,\sqrt 2)$
& $\frac{R}{4\pi}(2-\sqrt 2,-2+2\sqrt 2)$
& $-\frac{R}{2\pi}(-1+\sqrt 2)$
& $\frac{R}{2\pi}(1-\frac{\sqrt 2}{2})$
\\ \hline

$\{1,2\}$
& $-\frac{R}{2\pi}(\sqrt 2,0)$
& $\frac{\sqrt 2 R}{4\pi}(1,1)$
& $0$
& $\frac{\sqrt 2 R}{2\pi}$
\\ \hline

$\{2,3\}$
& $-\frac{R}{2\pi}(0,-\sqrt 2)$
& $\frac{\sqrt 2 R}{4\pi}(1,1)$
& $0$
& $\frac{\sqrt 2 R}{2\pi}$
\\ \hline

$\{3,4\}$
& $-\frac{R}{2\pi}(-\sqrt 2,0)$
& $\frac{\sqrt 2 R}{4\pi}(1,1)$
& $0$
& $\frac{\sqrt 2 R}{2\pi}$
\\ \hline

$\{1,4\}$
& $-\frac{R}{2\pi}(0,\sqrt 2)$
& $\frac{\sqrt 2 R}{4\pi}(1,1)$
& $0$
& $\frac{\sqrt 2 R}{2\pi}$
\\ \hline

$\{5,6\}$
& $-\frac{R}{2\pi}(1,1)$
& $\frac{R}{2\pi}(1,1)$
& $-\frac{R}{\pi}$
& $0$
\\ \hline

$\{3,5\}$
& $-\frac{R}{4\pi}(\sqrt 2,-2-\sqrt 2)$
& $\frac{R}{4\pi}(2+\sqrt 2,2+2\sqrt 2)$
& $-\frac{R}{2\pi}(1+\sqrt 2)$
& $\frac{R}{2\pi}(1+\frac{\sqrt 2}{2})$
\\ \hline

$\{3,6\}$
& $-\frac{R}{4\pi}(-2-\sqrt 2,\sqrt 2)$
& $\frac{R}{4\pi}(2+\sqrt 2,2+2\sqrt 2)$
& $-\frac{R}{2\pi}(1+\sqrt 2)$
& $\frac{R}{2\pi}(1+\frac{\sqrt 2}{2})$
\\ \hline
\end{tabular}
\caption{Computation of the different factors for different active constraints sets $I$ with the cost $\va c$ uniform on the sphere $R\cansph{1}$ centered on the origin of ray $R$} 
\end{table}

==> table/coef_infty_norm.tex <==
%!TEX root=../main.tex

\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
$I$ 
& \footnotesize{$\bprob{\va c \in -\cone\bp{W_{I}^\top}}$}
& \footnotesize{$\besp{\va c^\top |\va c \in -\cone\bp{W_{I}^\top}}$}
& $\coefc{I}^\top$
& $\tcoefc{I}^\top T$
& $\tcoefc{I}^\top h$
\\ \hline

$\{1,5\}$
& $\frc{1}{8}$
& $ -\frc{R}{3} (2,1)$
& $\frc{R}{24} (1,1)$
& $-\frc{R}{24}$
& $\frc{R}{24}$
\\ \hline

$\{2,5\}$
& $\frc{1}{8}$
& $\frc{-R}{3} (2,-1)$
& $\frc{R}{24} (1,1)$
& $-\frc{R}{24}$
& $\frc{R}{24}$
\\ \hline

$\{4,6\}$
& $\frc{1}{8}$
& $\frc{-R}{3} (-1,2)$
& $\frc{R}{24} (1,1)$
& $-\frc{R}{24}$
& $\frc{R}{24}$
\\ \hline


$\{1,6\}$
& $\frc{1}{8}$
& $\frc{-R}{3} (1,2)$
& $\frc{R}{24} (1,1)$
& $-\frc{R}{24}$
& $\frc{R}{24}$
\\ \hline

$\{1,2\}$
& $\frc{1}{4}$
& $-\frc{R}{3} (2,0)$
& $\frc{R}{12} (1,1)$
& $0$
& $\frc{R}{6}$
\\ \hline

$\{2,3\}$
& $\frc{1}{4}$
& $-\frc{R}{3} (0,-2)$
& $\frc{R}{12} (1,1)$
& $0$
& $\frc{R}{6}$
\\ \hline

$\{3,4\}$
& $\frc{1}{4}$
& $-\frc{R}{3} (-2,0)$
& $\frc{R}{12} (1,1)$
& $0$
& $\frc{R}{6}$
\\ \hline

$\{1,4\}$
& $\frc{1}{4}$
& $-\frc{R}{3} (0,2)$
& $\frc{R}{12} (1,1)$
& $0$
& $\frc{R}{6}$
\\ \hline

$\{5,6\}$
& $\frc{1}{4}$
& $-\frc{R}{2} (1,1)$
& $\frc{R}{8} (1,1)$
& $-\frc{R}{4}$
& $0$
\\ \hline

$\{3,5\}$
& $\frc{3}{8}$
& $-\frc{R}{9}(2,-5)$
& $\frc{R}{24}(5,7)$
& $-\frc{5R}{24}$
& $\frc{7R}{24}$
\\ \hline

$\{3,6\}$
& $\frc{3}{8}$
& $-\frc{R}{9}(-5,2)$
& $\frc{R}{24}(5,7)$
& $-\frc{5R}{24}$
& $\frc{7R}{24}$
\\ \hline
\end{tabular}
\caption{Computation of the different factors for different active constraints $I$ with the cost $\va c$ with density $d\PP(c) =\frac{\indi{\mynorm{c}_\infty \leq R}}{4R^2} dc$}
\end{table}


==> table/submatrix_inverse.tex <==
%!TEX root=../main.tex


\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
$I$ 
& 
$\{1,5\}$
& 

$\{2,5\}$
& 
$\{4,6\}$
& 
$\{1,6\}$
& 
$\{1,2\}$
& 
$\{2,3\}$
 \\ \hline

$W_I$
& 
$\begin{pmatrix}
1 & 1 \\
1 & 0\\
\end{pmatrix}$
&
$\begin{pmatrix}
1 & -1 \\
1 & 0\\
\end{pmatrix}$
&
$\begin{pmatrix}
-1 & 1 \\
0 & 1\\
\end{pmatrix}$
&
$\begin{pmatrix}
1 & 1 \\
0 & 1\\
\end{pmatrix}$
&
$\begin{pmatrix}
1 & 1 \\
1 & -1\\
\end{pmatrix}$
&
$\begin{pmatrix}
1 & -1 \\
-1 & -1
\end{pmatrix}$
\\ \hline


$(W_I)^{-1}$
& 
$\begin{pmatrix}
0 & 1 \\
1 & -1\\
\end{pmatrix}$
&
$\begin{pmatrix}
0 & 1 \\
-1 & 1\\
\end{pmatrix}$
&
$
\begin{pmatrix}
-1 & 1 \\
0 & 1\\
\end{pmatrix}
$
&
$\begin{pmatrix}
1 & -1 \\
0 & 1\\
\end{pmatrix}$
&
$\frac{1}{2}
\begin{pmatrix}
1 & 1 \\
1 & -1\\
\end{pmatrix}$
&
$\frac{1}{2}
\begin{pmatrix}
1 & -1 \\
-1 & -1\\
\end{pmatrix}$
\\ \hline
\end{tabular}



\begin{tabular}{|c|c|c|c|c|c|}
 \hline
$I$
& 
$\{3,4\}$
& 
$\{1,4\}$
& 
$\{5,6\}$
&
$\{3,5\}$
&
$\{3,6\}$ \\ \hline

$W_I$
&
$\begin{pmatrix}
-1 & -1 \\
-1 & 1
\end{pmatrix}$
&
$\begin{pmatrix}
1 & 1 \\
-1 & 1
\end{pmatrix}$
&
$\begin{pmatrix}
1 & 0 \\
0 & 1
\end{pmatrix}$
&
$\begin{pmatrix}
-1 & -1 \\
1 & 0
\end{pmatrix}$
&
$\begin{pmatrix}
-1 & -1 \\
0 & 1
\end{pmatrix}$
\\ \hline
$(W_I)^{-1}$
&
$
\frac{1}{2}
\begin{pmatrix}
-1 & -1 \\
-1 & 1
\end{pmatrix}$
&
$\frac{1}{2}\begin{pmatrix}
1 & -1 \\
1 & 1
\end{pmatrix}$
&
$\begin{pmatrix}
1 & 0 \\
0 & 1
\end{pmatrix}$
&
$\begin{pmatrix}
0 & 1 \\
-1 & -1 \\
\end{pmatrix}$
&
$\begin{pmatrix}
-1 & -1 \\
0 & 1
\end{pmatrix}$
\\ \hline
\end{tabular}
\caption{Submatrix and their inverse for each maximal active constraint sets}
\end{table}

==> tikz/polytope_fan_macro.tex <==
%




%

\coordinate (a) at (\ax,\ay);
\coordinate (b) at (\bx,\by);
\coordinate (c) at (\cx,\cy);
\coordinate (d) at (\dx,\dy);
\coordinate (e) at (\ex,\ey);


%
\coordinate (mab) at ($(a)!0.5!(b)$);
\coordinate (mbc) at ($(b)!0.5!(c)$);
\coordinate (mcd) at ($(c)!0.5!(d)$);
\coordinate (mde) at ($(d)!0.5!(e)$);
\coordinate (mea) at ($(e)!0.5!(a)$);

%
\pgfmathsetmacro\barx{1/5*(\ax+\bx+\cx+\dx+\ex)};
\pgfmathsetmacro\bary{1/5*(\ay+\by+\cy+\dy+\ey)};

%
\pgfmathsetmacro\nabx{\ay-\by};
\pgfmathsetmacro\nbcx{\by-\cy};
\pgfmathsetmacro\ncdx{\cy-\dy};
\pgfmathsetmacro\ndex{\dy-\ey};
\pgfmathsetmacro\neax{\ey-\ay};

\pgfmathsetmacro\naby{\bx-\ax};
\pgfmathsetmacro\nbcy{\cx-\bx};
\pgfmathsetmacro\ncdy{\dx-\cx};
\pgfmathsetmacro\ndey{\ex-\dx};
\pgfmathsetmacro\neay{\ax-\ex};

%
\coordinate (nab) at (\nabx,\naby);
\coordinate (nbc) at (\nbcx,\nbcy);
\coordinate (ncd) at (\ncdx,\ncdy);
\coordinate (nde) at (\ndex,\ndey);
\coordinate (nea) at (\neax,\neay);

%
\pgfmathsetmacro\angnab{atan2(\naby,\nabx)};
\pgfmathsetmacro\angnbc{atan2(\nbcy,\nbcx)};
\pgfmathsetmacro\angncd{atan2(\ncdy,\ncdx)};
\pgfmathsetmacro\angnde{atan2(\ndey,\ndex)};
\pgfmathsetmacro\angnea{atan2(\neay,\neax)};



%
\filldraw[fill=\colorpoly, draw=black] (a) -- (b) -- (c) -- (d) -- (e) --(a);

%
\filldraw[fill=\colorboundcone] (\barx,\bary) circle (0.17);

%
\draw[thick,->,\colorboundcone] (mab) to[offset=\lengthcone]++(nab);
\draw[thick,->,\colorboundcone] (mbc) to[offset=\lengthcone]++(nbc);
\draw[thick,->,\colorboundcone] (mcd) to[offset=\lengthcone]++(ncd);
\draw[thick,->,\colorboundcone] (mde) to[offset=\lengthcone]++(nde);
\draw[thick,->,\colorboundcone] (mea) to[offset=\lengthcone]++(nea);




%
%
\pgfmathparse{\angnea<\angnab}%
        \ifnum\pgfmathresult=1
                \pgfmathsetmacro\angnea{\angnea+360}%
        \fi 
\fill[\colorcone] ($(a) + (\angnea:\raycone)$) -- (a) -- ($(a)+ (\angnab:\raycone)$)  arc (\angnab:\angnea:\raycone);


\pgfmathparse{\angnab<\angnbc}%
        \ifnum\pgfmathresult=1
                \pgfmathsetmacro\angnab{\angnab+360}%
        \fi
\fill[\colorcone] ($(b) + (\angnab:\raycone)$) -- (b) -- ($(b)+ (\angnbc:\raycone)$)  arc (\angnbc:\angnab:\raycone);

\pgfmathparse{\angnbc<\angncd}%
        \ifnum\pgfmathresult=1
                \pgfmathsetmacro\angnbc{\angnbc+360}%
        \fi
\fill[\colorcone] ($(c) + (\angnbc:\raycone)$) -- (c) -- ($(c)+ (\angncd:\raycone)$)  arc (\angncd:\angnbc:\raycone);


\pgfmathparse{\angncd<\angnde}%
        \ifnum\pgfmathresult=1
                \pgfmathsetmacro\angncd{\angncd+360}%
        \fi
\fill[\colorcone] ($(d) + (\angncd:\raycone)$) -- (d) -- ($(d)+ (\angnde:\raycone)$)  arc (\angnde:\angncd:\raycone);

\pgfmathparse{\angnde<\angnea}%
        \ifnum\pgfmathresult=1
                \pgfmathsetmacro\angnde{\angnde+360}%
        \fi
\fill[\colorcone] ($(e) + (\angnde:\raycone)$) -- (e) -- ($(e)+ (\angnea:\raycone)$)  arc (\angnea:\angnde:\raycone);



%
\draw[thick,->,\colorboundcone] (a) to[offset=\lengthcone]++(nab);
\draw[thick,->,\colorboundcone] (b) to[offset=\lengthcone]++(nbc);
\draw[thick,->,\colorboundcone] (c) to[offset=\lengthcone]++(ncd);
\draw[thick,->,\colorboundcone] (d) to[offset=\lengthcone]++(nde);
\draw[thick,->,\colorboundcone] (e) to[offset=\lengthcone]++(nea);
\draw[thick,->,\colorboundcone] (b) to[offset=\lengthcone]++(nab);
\draw[thick,->,\colorboundcone] (c) to[offset=\lengthcone]++(nbc);
\draw[thick,->,\colorboundcone] (d) to[offset=\lengthcone]++(ncd);
\draw[thick,->,\colorboundcone] (e) to[offset=\lengthcone]++(nde);
\draw[thick,->,\colorboundcone] (a) to[offset=\lengthcone]++(nea);





%
%
%
%
%
%



